Formally Verified SAT-Based AI Planning

We present an executable formally verified SAT encoding of classical AI planning. We use the theorem prover Isabelle/HOL to perform the verification. We experimentally test the verified encoding and show that it can be used for reasonably sized standard planning benchmarks. We also use it as a reference to test a state-of-the-art SAT-based planner, showing that it sometimes falsely claims that problems have no solutions of certain lengths.

==> isabelle_snippets/edited_texs/__latexindent_temp.tex <==
%
\begin{isabellebody}%
\setisabellecontext{sas{\isacharunderscore}plus{\isacharunderscore}problem{\isacharunderscore}to{\isacharunderscore}strips{\isacharunderscore}problem{\isacharunderscore}def}%
%
\isadelimtheory
\ \ %
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\isadelimdocument
%
\endisadelimdocument
%
\isatagdocument
%
\endisatagdocument
{\isafolddocument}%
%
\isadelimdocument
%
\endisadelimdocument
%
\begin{isamarkuptext}%
%
\begin{isabelle}%
{\isasymphi}\ {\isasymPsi}\ \ {\isasymequiv}\ \ {\isasymlparr}\isanewline
\isaindent{\ }variables{\isacharunderscore}of\ {\isacharequal}\isanewline
\isaindent{var} concat\ {\isacharparenleft}map\ {\isacharparenleft}{\isasymlambda}v{\isachardot}\ map\ {\isacharparenleft}{\isasymlambda}as{\isachardot}\ as{\isacharparenright}\ {\isacharparenleft}possible{\isacharunderscore}assignments{\isacharunderscore}for\ {\isasymPsi}\ v{\isacharparenright}{\isacharparenright}\ {\isacharparenleft}{\isasymPsi}\isactrlsub {\isasymV}\isactrlsub {\isacharplus}{\isacharparenright}{\isacharparenright}{\isacharcomma}\isanewline
\isaindent{\ }operators{\isacharunderscore}of\ {\isacharequal}\ map\ {\isacharparenleft}{\isasymphi}\isactrlsub O{\isasyminverse}\ {\isasymPsi}{\isacharparenright}{\isacharparenleft}{\isasymPsi}\isactrlsub {\isasymO}\isactrlsub {\isacharplus}{\isacharparenright}{\isacharcomma}{\ }initial{\isacharunderscore}of\ {\isacharequal}\ {\isasymphi}\isactrlsub S\ {\isasymPsi}\ {\isasymPsi}\isactrlsub I\isactrlsub {\isacharplus}{\isacharcomma}\isanewline
\isaindent{\ }goal{\isacharunderscore}of\ {\isacharequal}\ {\isasymphi}\isactrlsub S\ {\isasymPsi}\ {\isasymPsi}\isactrlsub G\isactrlsub {\isacharplus}{\ }{\isasymrparr}%
\end{isabelle}%
\end{isamarkuptext}\isamarkuptrue%
%
\isadelimtheory
%
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\end{isabellebody}%
\endinput
%:%file=~/Documents/Workspace/Planning/papers/verified-SAT-plan/isabelle_snippets/sas_plus_problem_to_strips_problem_def.thy%:%
%:%6=1%:%


==> isabelle_snippets/edited_texs/are_operators_interfering_def.tex <==
%
\begin{isabellebody}%
\setisabellecontext{are{\isacharunderscore}operators{\isacharunderscore}interfering{\isacharunderscore}def}%
%
\isadelimtheory
%
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\begin{isamarkuptext}%
%
\begin{isabelle}%
are{\isacharunderscore}operators{\isacharunderscore}interfering\ op\isactrlsub {\isadigit{1}}\ op\isactrlsub {\isadigit{2}}\ {\isasymequiv}\isanewline
list{\isacharunderscore}ex\ {\isacharparenleft}{\isasymlambda}v{\isachardot}\ list{\isacharunderscore}ex\ {\isacharparenleft}{\isacharparenleft}{\isacharequal}{\isacharparenright}\ v{\isacharparenright}\ {\isacharparenleft}delete{\isacharunderscore}effects{\isacharunderscore}of\ op\isactrlsub {\isadigit{1}}{\isacharparenright}{\isacharparenright}\ {\isacharparenleft}precondition{\isacharunderscore}of\ op\isactrlsub {\isadigit{2}}{\isacharparenright}\ {\isasymor}\isanewline
list{\isacharunderscore}ex\ {\isacharparenleft}{\isasymlambda}v{\isachardot}\ list{\isacharunderscore}ex\ {\isacharparenleft}{\isacharparenleft}{\isacharequal}{\isacharparenright}\ v{\isacharparenright}\ {\isacharparenleft}precondition{\isacharunderscore}of\ op\isactrlsub {\isadigit{1}}{\isacharparenright}{\isacharparenright}\ {\isacharparenleft}delete{\isacharunderscore}effects{\isacharunderscore}of\ op\isactrlsub {\isadigit{2}}{\isacharparenright}%
\end{isabelle}%
\end{isamarkuptext}\isamarkuptrue%
%
\isadelimtheory
%
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\end{isabellebody}%
\endinput
%:%file=~/planning_tightness/papers/verified-SAT-plan/isabelle_snippets/are_operators_interfering_def.thy%:%


==> isabelle_snippets/edited_texs/assignment.tex <==
%
\begin{isabellebody}%
\setisabellecontext{assignment}%
%
\isadelimtheory
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
\isacommand{type{\isacharunderscore}synonym}\isamarkupfalse%
\ {\isacharparenleft}{\isacharprime}variable{\isacharcomma}\ {\isacharprime}domain{\isacharparenright}\ assignment\ {\isacharequal}\ {\isachardoublequoteopen}{\isacharprime}variable\ {\isasymtimes}\ {\isacharprime}domain{\isachardoublequoteclose}%
\isadelimtheory
%
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\end{isabellebody}%
\endinput
%:%file=~/planning_tightness/papers/verified-SAT-plan/isabelle_snippets/assignment.thy%:%
%:%6=1%:%
%:%17=6%:%
%:%18=6%:%


==> isabelle_snippets/edited_texs/ast_effect.tex <==
%
\begin{isabellebody}%
\setisabellecontext{ast{\isacharunderscore}effect}%
%
\isadelimtheory
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
\isacommand{type{\isacharunderscore}synonym}\isamarkupfalse%
\ ast{\isacharunderscore}effect\ {\isacharequal}\ {\isachardoublequoteopen}ast{\isacharunderscore}precond\ list\ {\isasymtimes}\ nat\ {\isasymtimes}\ nat\ option\ {\isasymtimes}\ nat{\isachardoublequoteclose}%
\isadelimtheory
%
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\end{isabellebody}%
\endinput
%:%file=~/planning_tightness/papers/verified-SAT-plan/isabelle_snippets/ast_effect.thy%:%
%:%6=1%:%
%:%17=6%:%
%:%18=6%:%


==> isabelle_snippets/edited_texs/ast_operator.tex <==
%
\begin{isabellebody}%
\setisabellecontext{ast{\isacharunderscore}operator}%
%
\isadelimtheory
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
\isacommand{type{\isacharunderscore}synonym}\isamarkupfalse%
\ ast{\isacharunderscore}operator\ {\isacharequal}\ {\isachardoublequoteopen}name\ {\isasymtimes}\ ast{\isacharunderscore}precond\ list\ {\isasymtimes}\ ast{\isacharunderscore}effect\ list\ {\isasymtimes}\ nat{\isachardoublequoteclose}%
\isadelimtheory
%
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\end{isabellebody}%
\endinput
%:%file=~/planning_tightness/papers/verified-SAT-plan/isabelle_snippets/ast_operator.thy%:%
%:%6=1%:%
%:%17=6%:%
%:%18=6%:%


==> isabelle_snippets/edited_texs/ast_problem.tex <==
%
\begin{isabellebody}%
\setisabellecontext{ast{\isacharunderscore}problem}%
%
\isadelimtheory
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
\isacommand{type{\isacharunderscore}synonym}\isamarkupfalse%
\ ast{\isacharunderscore}problem\ {\isacharequal}\ \isanewline
\ \ {\isachardoublequoteopen}ast{\isacharunderscore}variable{\isacharunderscore}section\ {\isasymtimes}\ ast{\isacharunderscore}initial{\isacharunderscore}state\ {\isasymtimes}\ ast{\isacharunderscore}goal\ {\isasymtimes}\ ast{\isacharunderscore}operator{\isacharunderscore}section{\isachardoublequoteclose}%
\isadelimtheory
%
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\end{isabellebody}%
\endinput
%:%file=~/planning_tightness/papers/verified-SAT-plan/isabelle_snippets/ast_problem.thy%:%
%:%6=1%:%
%:%17=6%:%
%:%18=6%:%
%:%19=7%:%


==> isabelle_snippets/edited_texs/ast_problem_abs_ast_initial_state_def.tex <==
%
\begin{isabellebody}%
\setisabellecontext{ast{\isacharunderscore}problem{\isacharunderscore}abs{\isacharunderscore}ast{\isacharunderscore}initial{\isacharunderscore}state{\isacharunderscore}def}%
%
\isadelimtheory
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\begin{isamarkuptext}%
%
\begin{isabelle}%
abs{\isacharunderscore}ast{\isacharunderscore}initial{\isacharunderscore}state\ P\ {\isasymequiv}\ map{\isacharunderscore}of\ {\isacharparenleft}zip\ {\isacharbrackleft}{\isadigit{0}}{\isachardot}{\isachardot}{\isacharless}{\isacharbar}astI\ P{\isacharbar}{\isacharbrackright}\ {\isacharparenleft}astI\ P{\isacharparenright}{\isacharparenright}%
\end{isabelle}%
\end{isamarkuptext}\isamarkuptrue%
%
\isadelimtheory
%
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\end{isabellebody}%
\endinput
%:%file=~/planning_tightness/papers/verified-SAT-plan/isabelle_snippets/ast_problem_abs_ast_initial_state_def.thy%:%
%:%6=1%:%


==> isabelle_snippets/edited_texs/ast_problem_abs_ast_operator_def.tex <==
%
\begin{isabellebody}%
\setisabellecontext{ast{\isacharunderscore}problem{\isacharunderscore}abs{\isacharunderscore}ast{\isacharunderscore}operator{\isacharunderscore}def}%
%
\isadelimtheory
%
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\isadelimdocument
%
\endisadelimdocument
%
\isatagdocument
%
\endisatagdocument
{\isafolddocument}%
%
\isadelimdocument
%
\endisadelimdocument
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\begin{isamarkuptext}%
%
\begin{isabelle}%
abs{\isacharunderscore}ast{\isacharunderscore}operator\ {\isasymequiv}\isanewline
{\isasymlambda}{\isacharparenleft}name{\isacharcomma}\ pres{\isacharcomma}\ effs{\isacharcomma}\ cost{\isacharparenright}{\isachardot}\isanewline
\isaindent{\ \ \ }{\isasymlparr}precondition{\isacharunderscore}of\ {\isacharequal}\ pres{\isacharcomma}\ effect{\isacharunderscore}of\ {\isacharequal}\ map\ {\isacharparenleft}{\isasymlambda}{\isacharparenleft}pres{\isacharcomma}\ v{\isacharcomma}\ imp{\isacharunderscore}pres{\isacharcomma}\ x{\isacharparenright}{\isachardot}\ {\isacharparenleft}v{\isacharcomma}\ x{\isacharparenright}{\isacharparenright}\ effs{\isasymrparr}%
\end{isabelle}%
\end{isamarkuptext}\isamarkuptrue%
%
\isadelimtheory
%
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\end{isabellebody}%
\endinput
%:%file=~/planning_tightness/papers/verified-SAT-plan/isabelle_snippets/ast_problem_abs_ast_operator_def.thy%:%


==> isabelle_snippets/edited_texs/ast_problem_decode_abs_plan_def.tex <==
%
\begin{isabellebody}%
\setisabellecontext{ast{\isacharunderscore}problem{\isacharunderscore}decode{\isacharunderscore}abs{\isacharunderscore}plan{\isacharunderscore}def}%
%
\isadelimtheory
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\begin{isamarkuptext}%
%
\begin{isabelle}%
\hspace{-2ex} decode{\isacharunderscore}abs{\isacharunderscore}plan\ {\isasymequiv}\ map\ {\isacharparenleft}fst\ {\isasymcirc}\ the\ {\isasymcirc}\ lookup{\isacharunderscore}action{\isacharparenright}\ {\isasymcirc}\ rem{\isacharunderscore}condless{\isacharunderscore}ops\ I%
\end{isabelle}%
\end{isamarkuptext}\isamarkuptrue%
%
\isadelimtheory
%
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\end{isabellebody}%
\endinput
%:%file=~/planning_tightness/papers/verified-SAT-plan/isabelle_snippets/ast_problem_decode_abs_plan_def.thy%:%
%:%6=1%:%


==> isabelle_snippets/edited_texs/ast_problem_execute_def.tex <==
%
\begin{isabellebody}%
\setisabellecontext{ast{\isacharunderscore}problem{\isacharunderscore}execute{\isacharunderscore}def}%
%
\isadelimtheory
%
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\isadelimdocument
%
\endisadelimdocument
%
\isatagdocument
%
\endisatagdocument
{\isafolddocument}%
%
\isadelimdocument
%
\endisadelimdocument
%
\isadelimdocument
%
\endisadelimdocument
%
\isatagdocument
%
\endisatagdocument
{\isafolddocument}%
%
\isadelimdocument
%
\endisadelimdocument
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimdocument
%
\endisadelimdocument
%
\isatagdocument
%
\endisatagdocument
{\isafolddocument}%
%
\isadelimdocument
%
\endisadelimdocument
%
\begin{isamarkuptext}%
%
\begin{isabelle}%
execute\ name\ s\ {\isasymequiv}\isanewline
case\ lookup{\isacharunderscore}operator\ name\ of\isanewline
Some\ {\isacharparenleft}name{\isacharcomma}\ pres{\isacharcomma}\ effs{\isacharcomma}\ cost{\isacharparenright}\ {\isasymRightarrow}\isanewline
\isaindent{\ \ }s\ {\isacharplus}{\isacharplus}\ map{\isacharunderscore}of\ {\isacharparenleft}map\ {\isacharparenleft}{\isasymlambda}{\isacharparenleft}pre{\isacharcomma}\ x{\isacharcomma}\ imp{\isacharunderscore}pre{\isacharcomma}\ v{\isacharparenright}{\isachardot}\ {\isacharparenleft}x{\isacharcomma}\ v{\isacharparenright}{\isacharparenright}\ {\isacharparenleft}filter\ {\isacharparenleft}eff{\isacharunderscore}enabled\ s{\isacharparenright}\ effs{\isacharparenright}{\isacharparenright}%
\end{isabelle}%
\end{isamarkuptext}\isamarkuptrue%
%
\isadelimdocument
%
\endisadelimdocument
%
\isatagdocument
%
\endisatagdocument
{\isafolddocument}%
%
\isadelimdocument
%
\endisadelimdocument
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimtheory
%
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\end{isabellebody}%
\endinput
%:%file=~/planning_tightness/papers/verified-SAT-plan/isabelle_snippets/ast_problem_execute_def.thy%:%


==> isabelle_snippets/edited_texs/ast_problem_path_to_simps.tex <==
%
\begin{isabellebody}%
\setisabellecontext{ast{\isacharunderscore}problem{\isacharunderscore}path{\isacharunderscore}to{\isacharunderscore}simps}%
%
\isadelimtheory
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\begin{isamarkuptext}%
%
\begin{isabelle}%
path{\isacharunderscore}to\ P\ s\ {\isacharbrackleft}{\isacharbrackright}\ s{\isacharprime}\ {\isacharequal}\ {\isacharparenleft}s{\isacharprime}\ {\isacharequal}\ s{\isacharparenright}\isasep\isanewline%
path{\isacharunderscore}to\ P\ s\ {\isacharparenleft}{\isasympi}\ {\isasymcdot}\ {\isasympi}s{\isacharparenright}\ s{\isacharprime}\ {\isacharequal}\ {\isacharparenleft}enabled\ P\ {\isasympi}\ s\ {\isasymand}\ path{\isacharunderscore}to\ P\ {\isacharparenleft}execute\ P\ {\isasympi}\ s{\isacharparenright}\ {\isasympi}s\ s{\isacharprime}{\isacharparenright}%
\end{isabelle}%
\end{isamarkuptext}\isamarkuptrue%
%
\isadelimtheory
%
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\end{isabellebody}%
\endinput
%:%file=~/planning_tightness/papers/verified-SAT-plan/isabelle_snippets/ast_problem_path_to_simps.thy%:%
%:%6=1%:%


==> isabelle_snippets/edited_texs/ast_problem_subsuming_states_def.tex <==
%
\begin{isabellebody}%
\setisabellecontext{ast{\isacharunderscore}problem{\isacharunderscore}subsuming{\isacharunderscore}states{\isacharunderscore}def}%
%
\isadelimtheory
%
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\begin{isamarkuptext}%
%
\begin{isabelle}%
subsuming{\isacharunderscore}states\ P\ pstate\ {\isasymequiv}\ {\isacharbraceleft}s\ {\isasymin}\ valid{\isacharunderscore}states\ P\ {\isacharbar}\ pstate\ {\isasymsubseteq}\isactrlsub m\ s{\isacharbraceright}%
\end{isabelle}%
\end{isamarkuptext}\isamarkuptrue%
%
\isadelimtheory
%
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\end{isabellebody}%
\endinput
%:%file=~/planning_tightness/papers/verified-SAT-plan/isabelle_snippets/ast_problem_subsuming_states_def.thy%:%


==> isabelle_snippets/edited_texs/ast_problem_valid_states_def.tex <==
%
\begin{isabellebody}%
\setisabellecontext{ast{\isacharunderscore}problem{\isacharunderscore}valid{\isacharunderscore}states{\isacharunderscore}def}%
%
\isadelimtheory
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\begin{isamarkuptext}%
%
\begin{isabelle}%
valid{\isacharunderscore}states\ P\ {\isasymequiv}\isanewline
{\isacharbraceleft}s\ {\isacharbar}\ dom\ s\ {\isacharequal}\ Dom\ P\ {\isasymand}\ {\isacharparenleft}{\isasymforall}x{\isasymin}Dom\ P{\isachardot}\ the\ {\isacharparenleft}s\ x{\isacharparenright}\ {\isasymin}\ range{\isacharunderscore}of{\isacharunderscore}var\ P\ x{\isacharparenright}{\isacharbraceright}%
\end{isabelle}%
\end{isamarkuptext}\isamarkuptrue%
%
\isadelimtheory
%
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\end{isabellebody}%
\endinput
%:%file=~/planning_tightness/papers/verified-SAT-plan/isabelle_snippets/ast_problem_valid_states_def.thy%:%
%:%6=1%:%


==> isabelle_snippets/edited_texs/ast_problem_wf_operator_def.tex <==
%
\begin{isabellebody}%
\setisabellecontext{ast{\isacharunderscore}problem{\isacharunderscore}wf{\isacharunderscore}operator{\isacharunderscore}def}%
%
\isadelimtheory
%
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\isadelimdocument
%
\endisadelimdocument
%
\isatagdocument
%
\endisatagdocument
{\isafolddocument}%
%
\isadelimdocument
%
\endisadelimdocument
%
\isadelimdocument
%
\endisadelimdocument
%
\isatagdocument
%
\endisatagdocument
{\isafolddocument}%
%
\isadelimdocument
%
\endisadelimdocument
%
\begin{isamarkuptext}%
%
\begin{isabelle}%
wf{\isacharunderscore}operator\ {\isasymequiv}\isanewline
{\isasymlambda}{\isacharparenleft}name{\isacharcomma}\ pres{\isacharcomma}\ effs{\isacharcomma}\ cost{\isacharparenright}{\isachardot}\isanewline
\isaindent{\ \ \ }wf{\isacharunderscore}partial{\isacharunderscore}state\ pres\ {\isasymand}\isanewline
\isaindent{\ \ \ }distinct\ {\isacharparenleft}map\ {\isacharparenleft}{\isasymlambda}{\isacharparenleft}name{\isacharcomma}\ x{\isacharcomma}\ imp{\isacharunderscore}pre{\isacharcomma}\ v{\isacharparenright}{\isachardot}\ x{\isacharparenright}\ effs{\isacharparenright}\ {\isasymand}\isanewline
\isaindent{\ \ \ }{\isacharparenleft}{\isasymforall}{\isacharparenleft}epres{\isacharcomma}\ x{\isacharcomma}\ vp{\isacharcomma}\ v{\isacharparenright}{\isasymin}set\ effs{\isachardot}\isanewline
\isaindent{\ \ \ {\isacharparenleft}\ \ \ }wf{\isacharunderscore}partial{\isacharunderscore}state\ epres\ {\isasymand}\ x\ {\isacharless}\ numVars\ {\isasymand} v\ {\isacharless}\ numVals\ x\ {\isasymand}\isanewline
\isaindent{\ \ \ {\isacharparenleft}\ \ \ }{\isacharparenleft}case\ vp\ of\ None\ {\isasymRightarrow}\ True\ {\isacharbar}\ Some\ v\ {\isasymRightarrow}\ v\ {\isacharless}\ numVals\ x{\isacharparenright}{\isacharparenright}%
\end{isabelle}%
\end{isamarkuptext}\isamarkuptrue%
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimdocument
%
\endisadelimdocument
%
\isatagdocument
%
\endisatagdocument
{\isafolddocument}%
%
\isadelimdocument
%
\endisadelimdocument
%
\isadelimdocument
%
\endisadelimdocument
%
\isatagdocument
%
\endisatagdocument
{\isafolddocument}%
%
\isadelimdocument
%
\endisadelimdocument
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimproof
%
\endisadelimproof
%
\isatagproof
%
\endisatagproof
{\isafoldproof}%
%
\isadelimproof
%
\endisadelimproof
%
\isadelimtheory
%
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\end{isabellebody}%
\endinput
%:%file=~/planning_tightness/papers/verified-SAT-plan/isabelle_snippets/ast_problem_wf_operator_def.thy%:%


==> isabelle_snippets/edited_texs/ast_problem_wf_partial_state_def.tex <==
%
\begin{isabellebody}%
\setisabellecontext{ast{\isacharunderscore}problem{\isacharunderscore}wf{\isacharunderscore}partial{\isacharunderscore}state{\isacharunderscore}def}%
%
\isadelimtheory
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\begin{isamarkuptext}%
%
\begin{isabelle}%
wf{\isacharunderscore}partial{\isacharunderscore}state\ P\ ps\ {\isasymequiv}\isanewline
distinct\ {\isacharparenleft}map\ fst\ ps{\isacharparenright}\ {\isasymand} {\isacharparenleft}{\isasymforall}{\isacharparenleft}x{\isacharcomma}\ v{\isacharparenright}{\isasymin}ps{\isachardot}\ x\ {\isacharless}\ numVars\ P\ {\isasymand}\ v\ {\isacharless}\ numVals\ P\ x{\isacharparenright}%
\end{isabelle}%
\end{isamarkuptext}\isamarkuptrue%
%
\isadelimtheory
%
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\end{isabellebody}%
\endinput
%:%file=~/planning_tightness/papers/verified-SAT-plan/isabelle_snippets/ast_problem_wf_partial_state_def.thy%:%
%:%6=1%:%


==> isabelle_snippets/edited_texs/ast_variable.tex <==
%
\begin{isabellebody}%
\setisabellecontext{ast{\isacharunderscore}variable}%
%
\isadelimtheory
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
\isacommand{type{\isacharunderscore}synonym}\isamarkupfalse%
\ ast{\isacharunderscore}variable\ {\isacharequal}\ {\isachardoublequoteopen}name\ {\isasymtimes}\ nat\ option\ {\isasymtimes}\ name\ list{\isachardoublequoteclose}%
\isadelimtheory
%
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\end{isabellebody}%
\endinput
%:%file=~/planning_tightness/papers/verified-SAT-plan/isabelle_snippets/ast_variable.thy%:%
%:%6=1%:%
%:%17=6%:%
%:%18=6%:%


==> isabelle_snippets/edited_texs/decode_complete.tex <==
%
\begin{isabellebody}%
\setisabellecontext{decode{\isacharunderscore}complete}%
%
\isadelimtheory
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\begin{isamarkuptext}%
%
\begin{isabelle}%
decode\ M\ h\ P\ {\isacharequal}\ Inr\ err\ {\isasymLongrightarrow}\isanewline
{\isasymnot}\ {\isacharparenleft}well{\isacharunderscore}formed\ P\ {\isasymand}\ {\isacharparenleft}{\isasymforall}$\pi${\isasymin}ast{\isasymdelta}\ P{\isachardot}\ consistent{\isacharunderscore}pres{\isacharunderscore}op\ $\pi${\isacharparenright}\ {\isasymand}\isanewline
\isaindent{{\isasymnot}\ {\isacharparenleft}}{\isacharparenleft}{\isasymforall}{\isasympi}{\isasymin}ast{\isasymdelta}\ P{\isachardot}\ is{\isacharunderscore}standard{\isacharunderscore}operator\ {\isasympi}{\isacharparenright}\ {\isasymand}\ dimacs{\isacharunderscore}model\ M\ {\isacharparenleft}encoding\ h\ P{\isacharparenright}{\isacharparenright}%
\end{isabelle}%
\end{isamarkuptext}\isamarkuptrue%
%
\isadelimtheory
%
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\end{isabellebody}%
\endinput
%:%file=~/planning_tightness/papers/verified-SAT-plan/isabelle_snippets/decode_complete.thy%:%
%:%6=1%:%


==> isabelle_snippets/edited_texs/decode_sound.tex <==
%
\begin{isabellebody}%
\setisabellecontext{decode{\isacharunderscore}sound}%
%
\isadelimtheory
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\begin{isamarkuptext}%
%
\begin{isabelle}%
decode\ M\ h\ P\ {\isacharequal}\ Inl\ $\pi$s\ {\isasymLongrightarrow}\ valid{\isacharunderscore}plan\ P\ $\pi$s%
\end{isabelle}%
\end{isamarkuptext}\isamarkuptrue%
%
\isadelimtheory
%
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\end{isabellebody}%
\endinput
%:%file=~/planning_tightness/papers/verified-SAT-plan/isabelle_snippets/decode_sound.thy%:%
%:%6=1%:%


==> isabelle_snippets/edited_texs/dimacs_model_def.tex <==
%
\begin{isabellebody}%
\setisabellecontext{dimacs{\isacharunderscore}model{\isacharunderscore}def}%
%
\isadelimtheory

\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\begin{isamarkuptext}%
%
\begin{isabelle}%
dimacs{\isacharunderscore}model\ ls\ cs\ {\isasymequiv}\ {\isacharparenleft}{\isasymforall}c{\isasymin}cs{\isachardot}\ {\isasymexists}l{\isasymin}ls{\isachardot}\ l\ {\isasymin}\ c{\isacharparenright}\ {\isasymand}\ distinct\ {\isacharparenleft}map\ dimacs{\isacharunderscore}lit{\isacharunderscore}to{\isacharunderscore}var\ ls{\isacharparenright}%
\end{isabelle}%
\end{isamarkuptext}\isamarkuptrue%
%
\isadelimtheory
%
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\end{isabellebody}%
\endinput
%:%file=~/planning_tightness/papers/verified-SAT-plan/isabelle_snippets/dimacs_model_def.thy%:%
%:%6=1%:%


==> isabelle_snippets/edited_texs/encode_complete.tex <==
%
\begin{isabellebody}%
\setisabellecontext{encode{\isacharunderscore}complete}%
%
\isadelimtheory
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\begin{isamarkuptext}%
%
\begin{isabelle}%
encode\ h\ P\ {\isacharequal}\ Inr\ err\ {\isasymLongrightarrow}\isanewline
{\isasymnot}\ {\isacharparenleft}well{\isacharunderscore}formed\ P\ {\isasymand}\isanewline
\isaindent{{\isasymnot}\ {\isacharparenleft}}{\isacharparenleft}{\isasymforall}$\pi${\isasymin}ast{\isasymdelta}\ P{\isachardot}\ consistent{\isacharunderscore}pres{\isacharunderscore}op\ $\pi${\isacharparenright}\ {\isasymand}\ {\isacharparenleft}{\isasymforall}$\pi${\isasymin}ast{\isasymdelta}\ P{\isachardot}\ is{\isacharunderscore}standard{\isacharunderscore}operator\ $\pi${\isacharparenright}{\isacharparenright}%
\end{isabelle}%
\end{isamarkuptext}\isamarkuptrue%
%
\isadelimtheory
%
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\end{isabellebody}%
\endinput
%:%file=~/planning_tightness/papers/verified-SAT-plan/isabelle_snippets/encode_complete.thy%:%
%:%6=1%:%


==> isabelle_snippets/edited_texs/encode_operator_precondition_def.tex <==
%
\begin{isabellebody}%
\setisabellecontext{encode{\isacharunderscore}operator{\isacharunderscore}precondition{\isacharunderscore}def}%
%
\isadelimtheory
\ \ %
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\begin{isamarkuptext}%
%
\begin{isabelle}%
encode{\isacharunderscore}operator{\isacharunderscore}precondition\ {\isasymPi}\ t\ op\ {\isasymequiv}\isanewline
\textsf{let}\ vs\ {\isacharequal}\ {\isasymPi}\isactrlsub {\isasymV}{\isacharsemicolon}\ ops\ {\isacharequal}\ {\isasymPi}\isactrlsub {\isasymO}\isanewline
\textsf{in}\ \isactrlbold {\isasymAnd}map\ {\isacharparenleft}{\isasymlambda}v{\isachardot}\ \isactrlbold {\isasymnot}\ {\isacharparenleft}Atom\ {\isacharparenleft}Operator\ t\ {\isacharparenleft}index\ ops\ op{\isacharparenright}{\isacharparenright}{\isacharparenright}\ \isactrlbold {\isasymor}\ Atom\ {\isacharparenleft}State\ t\ {\isacharparenleft}index\ vs\ v{\isacharparenright}{\isacharparenright}{\isacharparenright}\isanewline
\isaindent{\textsf{in}\ \isactrlbold {\isasymAnd}\ map}{\isacharparenleft}precondition{\isacharunderscore}of\ op{\isacharparenright}%
\end{isabelle}%
\end{isamarkuptext}\isamarkuptrue%
%
\isadelimtheory
%
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\end{isabellebody}%
\endinput
%:%file=~/planning_tightness/papers/verified-SAT-plan/isabelle_snippets/encode_operator_precondition_def.thy%:%
%:%6=1%:%


==> isabelle_snippets/edited_texs/encode_sound.tex <==
%
\begin{isabellebody}%
\setisabellecontext{encode{\isacharunderscore}sound}%
%
\isadelimtheory
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\begin{isamarkuptext}%
%
\begin{isabelle}%
valid{\isacharunderscore}plan\ P\ {\isasympi}s\ {\isasymand}\ {\isacharbar}{\isasympi}s{\isacharbar}\ {\isasymle}\ h\ {\isasymand}\ encode\ h\ P\ {\isacharequal}\ Inl\ $\Phi$\ {\isasymLongrightarrow}\ {\isasymexists}M{\isachardot}\ dimacs{\isacharunderscore}model\ M\ $\Phi$%
\end{isabelle}%
\end{isamarkuptext}\isamarkuptrue%
%
\isadelimtheory
%
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\end{isabellebody}%
\endinput
%:%file=~/planning_tightness/papers/verified-SAT-plan/isabelle_snippets/encode_sound.thy%:%
%:%6=1%:%


==> isabelle_snippets/edited_texs/name.tex <==
%
\begin{isabellebody}%
\setisabellecontext{name}%
%
\isadelimtheory

\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
\isacommand{type{\isacharunderscore}synonym}\isamarkupfalse%
\ name\ {\isacharequal}\ string%
\isadelimtheory
%
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\end{isabellebody}%
\endinput
%:%file=~/planning_tightness/papers/verified-SAT-plan/isabelle_snippets/name.thy%:%
%:%6=1%:%
%:%17=6%:%
%:%18=6%:%


==> isabelle_snippets/edited_texs/rem_effect_implicit_pres_simps.tex <==
%
\begin{isabellebody}%
\setisabellecontext{rem{\isacharunderscore}effect{\isacharunderscore}implicit{\isacharunderscore}pres{\isacharunderscore}simps}%
%
\isadelimtheory
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\begin{isamarkuptext}%
%
\begin{isabelle}%
rem{\isacharunderscore}effect{\isacharunderscore}implicit{\isacharunderscore}pres\ {\isacharparenleft}preconds{\isacharcomma}\ v{\isacharcomma}\ implicit{\isacharunderscore}pre{\isacharcomma}\ eff{\isacharparenright}\ {\isacharequal}\ {\isacharparenleft}preconds{\isacharcomma}\ v{\isacharcomma}\ None{\isacharcomma}\ eff{\isacharparenright}%
\end{isabelle}%
\end{isamarkuptext}\isamarkuptrue%
%
\isadelimtheory
%
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\end{isabellebody}%
\endinput
%:%file=~/planning_tightness/papers/verified-SAT-plan/isabelle_snippets/rem_effect_implicit_pres_simps.thy%:%
%:%6=1%:%


==> isabelle_snippets/edited_texs/rem_implicit_pres_simps.tex <==
%
\begin{isabellebody}%
\setisabellecontext{rem{\isacharunderscore}implicit{\isacharunderscore}pres{\isacharunderscore}simps}%
%
\isadelimtheory
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\begin{isamarkuptext}%
%
\begin{isabelle}%
rem{\isacharunderscore}implicit{\isacharunderscore}pres\ {\isacharparenleft}name{\isacharcomma}\ pres{\isacharcomma}\ effs{\isacharcomma}\ cost{\isacharparenright}\ {\isacharequal}\isanewline
{\isacharparenleft}name{\isacharcomma}\ implicit{\isacharunderscore}pres\ effs\ \isacharat\ pres{\isacharcomma}\ map\ rem{\isacharunderscore}effect{\isacharunderscore}implicit{\isacharunderscore}pres\ effs{\isacharcomma}\ cost{\isacharparenright}%
\end{isabelle}%
\end{isamarkuptext}\isamarkuptrue%
%
\isadelimtheory
%
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\end{isabellebody}%
\endinput
%:%file=~/planning_tightness/papers/verified-SAT-plan/isabelle_snippets/rem_implicit_pres_simps.thy%:%
%:%6=1%:%


==> isabelle_snippets/edited_texs/sas_plus_operator.tex <==
%
\begin{isabellebody}%
\setisabellecontext{sas{\isacharunderscore}plus{\isacharunderscore}operator}%
%
\isadelimtheory
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
\isacommand{record}\isamarkupfalse%
\ \ {\isacharparenleft}{\isacharprime}variable{\isacharcomma}\ {\isacharprime}domain{\isacharparenright}\ sas{\isacharunderscore}plus{\isacharunderscore}operator\ {\isacharequal}\ \isanewline
\ \ precondition{\isacharunderscore}of\ {\isacharcolon}{\isacharcolon}\ {\isachardoublequoteopen}{\isacharparenleft}{\isacharprime}variable{\isacharcomma}\ {\isacharprime}domain{\isacharparenright}\ assignment\ list{\isachardoublequoteclose}\ \isanewline
\ \ effect{\isacharunderscore}of\ {\isacharcolon}{\isacharcolon}\ {\isachardoublequoteopen}{\isacharparenleft}{\isacharprime}variable{\isacharcomma}\ {\isacharprime}domain{\isacharparenright}\ assignment\ list{\isachardoublequoteclose}%
\isadelimtheory
%
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\end{isabellebody}%
\endinput
%:%file=~/planning_tightness/papers/verified-SAT-plan/isabelle_snippets/sas_plus_operator.thy%:%
%:%6=1%:%
%:%17=6%:%
%:%18=6%:%
%:%19=7%:%
%:%20=8%:%


==> isabelle_snippets/edited_texs/sas_plus_problem_to_strips_problem_def.tex <==
%
\begin{isabellebody}%
\setisabellecontext{sas{\isacharunderscore}plus{\isacharunderscore}problem{\isacharunderscore}to{\isacharunderscore}strips{\isacharunderscore}problem{\isacharunderscore}def}%
%
\isadelimtheory
\ \ %
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\isadelimdocument
%
\endisadelimdocument
%
\isatagdocument
%
\endisatagdocument
{\isafolddocument}%
%
\isadelimdocument
%
\endisadelimdocument
%
\begin{isamarkuptext}%
%
\begin{isabelle}%
{\isasymphi}\ {\isasymPsi}\ \ {\isasymequiv}\ \ {\isasymlparr}\isanewline
\isaindent{\ }variables{\isacharunderscore}of\ {\isacharequal}\isanewline
\isaindent{var} concat\ {\isacharparenleft}map\ {\isacharparenleft}{\isasymlambda}v{\isachardot}\ map\ {\isacharparenleft}{\isasymlambda}as{\isachardot}\ as{\isacharparenright}\ {\isacharparenleft}possible{\isacharunderscore}assignments{\isacharunderscore}for\ {\isasymPsi}\ v{\isacharparenright}{\isacharparenright}\ {\isacharparenleft}{\isasymPsi}\isactrlsub {\isasymV}\isactrlsub {\isacharplus}{\isacharparenright}{\isacharparenright}{\isacharcomma}\isanewline
\isaindent{\ }operators{\isacharunderscore}of\ {\isacharequal}\ map\ {\isacharparenleft}{\isasymphi}\isactrlsub O{\isasyminverse}\ {\isasymPsi}{\isacharparenright}{\isacharparenleft}{\isasymPsi}\isactrlsub {\isasymO}\isactrlsub {\isacharplus}{\isacharparenright}{\isacharcomma}{\ }initial{\isacharunderscore}of\ {\isacharequal}\ {\isasymphi}\isactrlsub S\ {\isasymPsi}\ {\isasymPsi}\isactrlsub I\isactrlsub {\isacharplus}{\isacharcomma}\isanewline
\isaindent{\ }goal{\isacharunderscore}of\ {\isacharequal}\ {\isasymphi}\isactrlsub S\ {\isasymPsi}\ {\isasymPsi}\isactrlsub G\isactrlsub {\isacharplus}{\ }{\isasymrparr}%
\end{isabelle}%
\end{isamarkuptext}\isamarkuptrue%
%
\isadelimtheory
%
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\end{isabellebody}%
\endinput
%:%file=~/Documents/Workspace/Planning/papers/verified-SAT-plan/isabelle_snippets/sas_plus_problem_to_strips_problem_def.thy%:%
%:%6=1%:%


==> isabelle_snippets/edited_texs/sasp_op_to_strips_def.tex <==
%
\begin{isabellebody}%
\setisabellecontext{sasp{\isacharunderscore}op{\isacharunderscore}to{\isacharunderscore}strips{\isacharunderscore}def}%
%
\isadelimtheory
%
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\isadelimdocument
%
\endisadelimdocument
%
\isatagdocument
%
\endisatagdocument
{\isafolddocument}%
%
\isadelimdocument
%
\endisadelimdocument
%
\isadelimdocument
%
\endisadelimdocument
%
\isatagdocument
%
\endisatagdocument
{\isafolddocument}%
%
\isadelimdocument
%
\endisadelimdocument
%
\begin{isamarkuptext}%
%
\begin{isabelle}%
{\isasymphi}\isactrlsub O\ {\isasymPsi}\ op\ {\isasymequiv}\ \ {\isasymlparr}\isanewline
\isaindent{\ }precondition{\isacharunderscore}of\ {\isacharequal}\ precondition{\isacharunderscore}of\ op{\isacharcomma}\isanewline
\isaindent{\ }add{\isacharunderscore}effects{\isacharunderscore}of\ {\isacharequal}\ effect{\isacharunderscore}of\ op{\isacharcomma}\isanewline
\isaindent{\ }delete{\isacharunderscore}effects{\isacharunderscore}of\ {\isacharequal}\ concat\isanewline
\isaindent{\ {\isacharparenleft}\ }{\isacharparenleft}map\ {\isacharparenleft}{\isasymlambda}{\isacharparenleft}v{\isacharcomma}\ a{\isacharparenright}{\isachardot}\ map\ {\isacharparenleft}Pair\ v{\isacharparenright}\ {\isacharparenleft}filter\ {\isacharparenleft}{\isacharparenleft}{\isasymnoteq}{\isacharparenright}\ a{\isacharparenright}\ {\isacharparenleft}the\ {\isacharparenleft}range{\isacharunderscore}of\ {\isasymPsi}\ v{\isacharparenright}{\isacharparenright}{\isacharparenright}{\isacharparenright}\ {\isacharparenleft}effect{\isacharunderscore}of\ op{\isacharparenright}{\isacharparenright}{\isasymrparr}%
\end{isabelle}%
\end{isamarkuptext}\isamarkuptrue%
%
\isadelimtheory
%
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\end{isabellebody}%
\endinput
%:%file=~/Documents/Workspace/Planning/papers/verified-SAT-plan/isabelle_snippets/sasp_op_to_strips_def.thy%:%


==> isabelle_snippets/edited_texs/serial_sas_plus_equivalent_to_serial_strips.tex <==
%
\begin{isabellebody}%
\setisabellecontext{serial{\isacharunderscore}sas{\isacharunderscore}plus{\isacharunderscore}equivalent{\isacharunderscore}to{\isacharunderscore}serial{\isacharunderscore}strips}%
%
\isadelimtheory
%
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\begin{isamarkuptext}%
%
\begin{isabelle}%
is{\isacharunderscore}valid{\isacharunderscore}problem{\isacharunderscore}sas{\isacharunderscore}plus\ {\isasymPsi}\ {\isasymand}\ is{\isacharunderscore}serial{\isacharunderscore}solution{\isacharunderscore}for{\isacharunderscore}problem\ {\isasymPsi}\ {\isasympsi}\ {\isasymLongrightarrow}\isanewline
is{\isacharunderscore}serial{\isacharunderscore}solution{\isacharunderscore}for{\isacharunderscore}problem\ {\isacharparenleft}{\isasymphi}\ {\isasymPsi}\ {\isacharparenright}\ {\isacharparenleft}map\ {\isacharparenleft}{\isasymphi}\isactrlsub O\ {\isasymPsi}{\isacharparenright}\ {\isasympsi}{\isacharparenright}%
\end{isabelle}%
\end{isamarkuptext}\isamarkuptrue%
%
\isadelimtheory
%
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\end{isabellebody}%
\endinput
%:%file=~/planning_tightness/papers/verified-SAT-plan/isabelle_snippets/serial_sas_plus_equivalent_to_serial_strips.thy%:%


==> isabelle_snippets/edited_texs/serial_strips_equivalent_to_serial_sas_plus.tex <==
%
\begin{isabellebody}%
\setisabellecontext{serial{\isacharunderscore}strips{\isacharunderscore}equivalent{\isacharunderscore}to{\isacharunderscore}serial{\isacharunderscore}sas{\isacharunderscore}plus}%
%
\isadelimtheory
%
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\begin{isamarkuptext}%
%
\begin{isabelle}%
is{\isacharunderscore}valid{\isacharunderscore}problem{\isacharunderscore}sas{\isacharunderscore}plus\ {\isasymPsi}\ {\isasymand}\ is{\isacharunderscore}serial{\isacharunderscore}solution{\isacharunderscore}for{\isacharunderscore}problem\ {\isacharparenleft}{\isasymphi}\ {\isasymPsi}\ {\isacharparenright}\ {\isasympi}\ {\isasymLongrightarrow}\isanewline
is{\isacharunderscore}serial{\isacharunderscore}solution{\isacharunderscore}for{\isacharunderscore}problem\ {\isasymPsi}\ {\isacharparenleft}map\ {\isacharparenleft}{\isasymphi}\isactrlsub O{\isasyminverse}\ {\isasymPsi}{\isacharparenright}\ {\isasympi}{\isacharparenright}%
\end{isabelle}%
\end{isamarkuptext}\isamarkuptrue%
%
\isadelimtheory
%
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\end{isabellebody}%
\endinput
%:%file=~/Documents/Workspace/Planning/papers/verified-SAT-plan/isabelle_snippets/serial_strips_equivalent_to_serial_sas_plus.thy%:%


==> isabelle_snippets/edited_texs/state.tex <==
%
\begin{isabellebody}%
\setisabellecontext{state}%
%
\isadelimtheory
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
\isacommand{type{\isacharunderscore}synonym}\isamarkupfalse%
\ {\isacharparenleft}{\isacharprime}variable{\isacharcomma}\ {\isacharprime}domain{\isacharparenright}\ state\ {\isacharequal}\ {\isachardoublequoteopen}{\isacharprime}variable\ {\isasymrightharpoonup}\ {\isacharprime}domain{\isachardoublequoteclose}%
\isadelimtheory
%
\endisadelimtheory
%
\isatagtheory
%
\endisatagtheory
{\isafoldtheory}%
%
\isadelimtheory
%
\endisadelimtheory
%
\end{isabellebody}%
\endinput
%:%file=~/planning_tightness/papers/verified-SAT-plan/isabelle_snippets/state.thy%:%
%:%6=1%:%
%:%17=6%:%
%:%18=6%:%

